Video Recognition in Portrait Mode

The creation of new datasets often presents new challenges for video recognition and can inspire novel ideas while addressing these challenges. While existing datasets mainly comprise landscape mode videos, our paper seeks to introduce portrait mode videos to the research community and highlight the unique challenges associated with this video format. With the growing popularity of smartphones and social media applications, recognizing portrait mode videos is becoming increasingly important. To this end, we have developed the first dataset dedicated to portrait mode video recognition, namely PortraitMode-400. The taxonomy of PortraitMode-400 was constructed in a data-driven manner, comprising 400 fine-grained categories, and rigorous quality assurance was implemented to ensure the accuracy of human annotations. In addition to the new dataset, we conducted a comprehensive analysis of the impact of video format (portrait mode versus landscape mode) on recognition accuracy and spatial bias due to the different formats. Furthermore, we designed extensive experiments to explore key aspects of portrait mode video recognition, including the choice of data augmentation, evaluation procedure, the importance of temporal information, and the role of audio modality. Building on the insights from our experimental results and the introduction of PortraitMode-400, our paper aims to inspire further research efforts in this emerging research area.

==> tables/audio_modality.tex <==

\setlength{\tabcolsep}{2.0mm}
\begin{tabular}
{c | c | c}
\toprule

Model & Modality & Top1-Acc.\\
\arrayrulecolor{white}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{white}\cline{3-5}
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{K400} & V & 75.6 \\
\arrayrulecolor{white}\cline{2-3}
\arrayrulecolor{white}\cline{2-3}
\arrayrulecolor{black}\cline{2-3}
\arrayrulecolor{white}\cline{2-3}
\arrayrulecolor{white}\cline{2-3}
                       & V+A & 77.0 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{3Massiv} & V & 53.79 \\
\arrayrulecolor{white}\cline{2-3}
\arrayrulecolor{white}\cline{2-3}
\arrayrulecolor{black}\cline{2-3}
\arrayrulecolor{white}\cline{2-3}
\arrayrulecolor{white}\cline{2-3}
                       & V+A & \textcolor{red}{25.27} \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{\textcolor{red}{Ours}} & V & 74.58 \\
\arrayrulecolor{white}\cline{2-3}
\arrayrulecolor{white}\cline{2-3}
\arrayrulecolor{black}\cline{2-3}
\arrayrulecolor{white}\cline{2-3}
\arrayrulecolor{white}\cline{2-3}
                       & V+A & \textcolor{red}{62.45} \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline



\end{tabular}

==> tables/main_crop_recipe_3massiv.tex <==
\setlength{\tabcolsep}{2.2mm}
\begin{tabular}
{c | c | c | c c}
\toprule
\multirow{3}{*}{Method} & \multirow{3}{*}{Inference} & \multicolumn{3}{c}{Training} \\
\arrayrulecolor{white}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{white}\cline{3-5}
 & & Random & \multicolumn{2}{c}{Shorter-side} \\
\arrayrulecolor{white}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{white}\cline{3-5}
 & & Square & 1:1 & 9:6 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{1}{*}{Uniformer} & 1:1 & 44.7 & 46.2 & 47.9 \\
                        %   & 9:6 & 45.0 &  & 49.18 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{1}{*}{MViTv2}    & 1:1 & 50.4 & 50.8 & 52.4 \\
                        %   & 9:6 &   &   &   \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline



\end{tabular}

==> tables/main_crop_recipe_dyo_v2.tex <==

\setlength{\tabcolsep}{2.2mm}
\begin{tabular}
{c | c | c | c c}
\toprule
\multirow{3}{*}{Method} & \multirow{3}{*}{Inference} & \multicolumn{3}{c}{Training} \\
\arrayrulecolor{white}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{white}\cline{3-5}
 & & Random & \multicolumn{2}{c}{Shorter-side} \\
\arrayrulecolor{white}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{white}\cline{3-5}
 & & Square & 1:1 & 9:6 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{1}{*}{Uniformer} & 1:1 & 50.2 & 51.4 & 52.2 \\
                        %   & 9:6 & 45.0 &  & 49.18 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{1}{*}{MViTv2}    & 1:1 & 53.3 & 53.9 & 53.6 \\
                        %   & 9:6 &   &   &   \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline



\end{tabular}

==> tables/main_crop_recipe_s100.tex <==

\setlength{\tabcolsep}{1.6mm}
% \tablestyle{2pt}{1.05}
\begin{tabular}
{c | c | c c | c}

% shorter - single crop test
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Train set} & \multicolumn{2}{c}{Top-1 Acc.} & \multirow{2}{*}{GFLOPs\x views}\\
\arrayrulecolor{white}\cline{3-4}
\arrayrulecolor{black}\cline{3-4}
\arrayrulecolor{black}\cline{3-4}
\arrayrulecolor{white}\cline{3-4}
  & & PM & LM & \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
% \multirow{2}{*}{X3D-M} & PM & 53.09 & 43.6 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
%                        & LM & 45.29 & 44.82 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
\multirow{2}{*}{X3D-M\cite{feichtenhofer2020x3d}}& PM  & 52.0 & 41.2 & 4.9$\times$3$\times$10 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
                     & LM & 44.5 & 43.5 & 4.9$\times$3$\times$10 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
% \multirow{2}{*}{Uniformer-S} & PM & 40.50 & 34.19 \\
% \multirow{2}{*}{Uniformer-S} & PM & 39.70 & 34.08 \\
\multirow{2}{*}{Uniformer-S\cite{li2022uniformer}} & PM  & 42.0 & 36.2 & 41.8$\times$1$\times$4 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
                                 % & LM & 37.88 & 38.67 \\
                                 % & LM & 37.08 & 38.10 \\
                       & LM & 40.1 & 40.8 &41.8$\times$1$\times$4 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{MViTv2-S\cite{li2022mvitv2}} & PM & 41.0 & 35.7 & 64$\times$1$\times$5 \\
% \multirow{2}{*}{MViTv2-S}    & PM & 36.94 & 32.16 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
                        & LM & 33.7 & 36.3 & 64$\times$1$\times$5\\
                                 % & LM & 35.60 & 37.49 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline


% \toprule
% \multirow{2}{*}{Method} & \multirow{2}{*}{Train set} & \multicolumn{2}{c}{Top-1 Acc.} \\
% \arrayrulecolor{white}\cline{3-4}
% \arrayrulecolor{black}\cline{3-4}
% \arrayrulecolor{black}\cline{3-4}
% \arrayrulecolor{white}\cline{3-4}
%  & & PM & LM \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% % \multirow{2}{*}{X3D-M} & PM & 53.09 & 43.6 \\
% % \arrayrulecolor{white}\cline{2-4}
% % \arrayrulecolor{black}\cline{2-4}
% % \arrayrulecolor{white}\cline{2-4}
% %                        & LM & 45.29 & 44.82 \\
% % \arrayrulecolor{white}\hline
% % \arrayrulecolor{black}\hline
% % \arrayrulecolor{white}\hline
% \multirow{2}{*}{X3D-M} & PM & 51.97 & 41.20 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
%                        & LM & 44.52 & 43.50 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% \multirow{2}{*}{Uniformer-S} & PM & 40.50 & 34.19 \\
% % \multirow{2}{*}{Uniformer-S} & PM & 39.70 & 34.08 \\
% % \multirow{2}{*}{Uniformer-S} & PM & 41.98 & 36.23 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
%                                  & LM & 37.88 & 38.67 \\
%                                  % & LM & 37.08 & 38.10 \\
%                                  % & LM & 40.13 & 40.76 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% \multirow{2}{*}{MViTv2-S}    & PM & 41.04 & 35.73 \\
% % \multirow{2}{*}{MViTv2-S}    & PM & 36.94 & 32.16 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
%                                  & LM & 33.71 & 36.34 \\
%                                  % & LM & 35.60 & 37.49 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline

\end{tabular}

==> tables/main_crop_s100_new_bak.tex <==

\setlength{\tabcolsep}{1.3mm}
% \tablestyle{2pt}{1.05}
\small
\begin{tabular}
{l | c | c | c | c | c}

% shorter - single crop test
% \toprule
% \multirow{2}{*}{Method} & \multirow{2}{*}{Train set} & \multicolumn{2}{c}{Top-1 Acc.} & \multirow{2}{*}{GFLOPs\x views}\\
\multicolumn{1}{c|}{Model} & Train  & Val &   Top-1  & Top-5  & GFLOPs\x views  \\
\shline
\multirow{4}{*}{X3D-M\cite{feichtenhofer2020x3d}}& \multirow{2}{*}{PM}  & \cellcolor{gray!20} PM & \cellcolor{gray!20} \textbf{52.0} & \cellcolor{gray!20} 41.2 & \cellcolor{gray!20} 4.9$\times$3$\times$10 \\
 &   & LM & 41.2 & 41.2 & 4.9$\times$3$\times$10 \\
% \arrayrulecolor{white}\cline{2-6}
\arrayrulecolor{black}\cline{2-6}
% \arrayrulecolor{white}\cline{2-6}
 & \multirow{2}{*}{LM}  & PM & \textbf{44.5} & 41.2 & 4.9$\times$3$\times$10 \\
 &   & LM & 43.5 & 41.2 & 4.9$\times$3$\times$10 \\
\hline
% \rowcolor{gray!20} 
\multirow{4}{*}{Uniformer-S\cite{li2022uniformer}} & \multirow{2}{*}{PM} & \cellcolor{gray!20} PM  & \cellcolor{gray!20} \textbf{42.0} & \cellcolor{gray!20} 36.2 &\cellcolor{gray!20}  41.8$\times$1$\times$4 \\
 &   & LM  & 36.2 & 36.2 & 41.8$\times$1$\times$4 \\
\arrayrulecolor{black}\cline{2-6}
 & \multirow{2}{*}{LM} & PM  & 40.1 & 36.2 & 41.8$\times$1$\times$4 \\
 &   & LM  & \textbf{40.8} & 36.2 & 41.8$\times$1$\times$4 \\
\hline

\multirow{4}{*}{MViTv2-S\cite{li2022mvitv2}} & \multirow{2}{*}{PM} & \cellcolor{gray!20} PM & \cellcolor{gray!20} \textbf{41.0} & \cellcolor{gray!20}  35.7 & \cellcolor{gray!20}  64$\times$1$\times$5 \\
% \multirow{2}{*}{MViTv2-S}    & PM & 36.94 & 32.16 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
                       &   & LM & 35.7 & 36.3 & 64$\times$1$\times$5\\
\arrayrulecolor{black}\cline{2-6}
                        & \multirow{2}{*}{LM} & PM & 33.7 & 36.3 & 64$\times$1$\times$5\\
                        &   & LM & \textbf{36.3} & 36.3 & 64$\times$1$\times$5\\
                                 % & LM & 35.60 & 37.49 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline


% \toprule
% \multirow{2}{*}{Method} & \multirow{2}{*}{Train set} & \multicolumn{2}{c}{Top-1 Acc.} \\
% \arrayrulecolor{white}\cline{3-4}
% \arrayrulecolor{black}\cline{3-4}
% \arrayrulecolor{black}\cline{3-4}
% \arrayrulecolor{white}\cline{3-4}
%  & & PM & LM \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% % \multirow{2}{*}{X3D-M} & PM & 53.09 & 43.6 \\
% % \arrayrulecolor{white}\cline{2-4}
% % \arrayrulecolor{black}\cline{2-4}
% % \arrayrulecolor{white}\cline{2-4}
% %                        & LM & 45.29 & 44.82 \\
% % \arrayrulecolor{white}\hline
% % \arrayrulecolor{black}\hline
% % \arrayrulecolor{white}\hline
% \multirow{2}{*}{X3D-M} & PM & 51.97 & 41.20 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
%                        & LM & 44.52 & 43.50 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% \multirow{2}{*}{Uniformer-S} & PM & 40.50 & 34.19 \\
% % \multirow{2}{*}{Uniformer-S} & PM & 39.70 & 34.08 \\
% % \multirow{2}{*}{Uniformer-S} & PM & 41.98 & 36.23 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
%                                  & LM & 37.88 & 38.67 \\
%                                  % & LM & 37.08 & 38.10 \\
%                                  % & LM & 40.13 & 40.76 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% \multirow{2}{*}{MViTv2-S}    & PM & 41.04 & 35.73 \\
% % \multirow{2}{*}{MViTv2-S}    & PM & 36.94 & 32.16 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
%                                  & LM & 33.71 & 36.34 \\
%                                  % & LM & 35.60 & 37.49 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline

\end{tabular}

==> tables/patch_shape_MViTv2.tex <==

\setlength{\tabcolsep}{2.2mm}
\begin{tabular}
{c | c | c | c | c c}
\toprule
\multirow{4}{*}{Dataset} & \multirow{4}{*}{Inference} & \multicolumn{4}{c}{Training} \\
\arrayrulecolor{white}\cline{3-6}
\arrayrulecolor{black}\cline{3-6}
\arrayrulecolor{black}\cline{3-6}
\arrayrulecolor{white}\cline{3-6}
 & & Random & \multicolumn{3}{c}{Shorter-side} \\
\arrayrulecolor{white}\cline{3-6}
\arrayrulecolor{black}\cline{3-6}
\arrayrulecolor{black}\cline{3-6}
\arrayrulecolor{white}\cline{3-6}
 & & Square & 1:1 & \multicolumn{2}{c}{9:6} \\
\arrayrulecolor{white}\cline{3-6}
\arrayrulecolor{black}\cline{3-6}
\arrayrulecolor{black}\cline{3-6}
\arrayrulecolor{white}\cline{3-6}
 & & P 1:1 & P 1:1 & P 1:1 & P 9:6 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{3Massiv} & 1:1 & 50.4 & 50.8 & 52.4 & 50.8 \\
                          & 9:6 &  & 51.4 &   & 51.9 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{DYO-v2}    & 1:1 & 54.00 & 54.7 & 54.4 & 54.0 \\
                          & 9:6 & 54.0 & 54.3 & 54.7 & 54.8 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{1}{*}{S100}    & 1:1 & 38.5 & 40.0 & 45.2 & 46.2 \\
                        %   & 9:6 & 54.0 & 54.3 & 54.7 & 54.8 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline



\end{tabular}

==> tables/resizing_sampling.tex <==

\setlength{\tabcolsep}{2.2mm}
\begin{tabular}
{c | c | c c}
\toprule
\multirow{2}{*}{Data} & \multirow{2}{*}{Model} & \multicolumn{2}{c}{Recipes} \\
\arrayrulecolor{white}\cline{3-4}
\arrayrulecolor{black}\cline{3-4}
\arrayrulecolor{black}\cline{3-4}
\arrayrulecolor{white}\cline{3-4}
 & & Default & Shorter-side \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{S100-PM} & Uniformer-S & 40.5 & 42.18 \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                       & MViTv2-S & 36.94 & 41.04 \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                       & \textcolor{red}{X3D-M} & xx & xx \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{3Massiv} & Uniformer-S & 42.76 & 44.75 \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                          & MViTv2-S & 50.36 & 52.08 \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                       & \textcolor{red}{X3D-M} & xx & xx \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{\textcolor{red}{Ours}} & Uniformer-S & 70.82 & 71.77 \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                          & MViTv2-S & 80.70 & 80.68 \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                       & \textcolor{red}{X3D-M} & xx & xx \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline



\end{tabular}

==> tables/resizing_sampling_recipe_new_style.tex <==

\setlength{\tabcolsep}{1.8mm}
\begin{tabular}
{c | c | c| c c}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Data} & \multicolumn{2}{c}{Recipes} \\
\arrayrulecolor{white}\cline{3-4}
\arrayrulecolor{black}\cline{3-4}
\arrayrulecolor{black}\cline{3-4}
\arrayrulecolor{white}\cline{3-4}
 & & Inception-style & Shorter-side \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{X3D-M\cite{feichtenhofer2020x3d}} & S100-PM & \textbf{54.2} & 52.0 \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                          & 3Massiv & \textbf{53.7} & 52.6 \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                       & \abbrdataset & \textbf{61.7} & 61.2 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{Uniformer-S\cite{li2022uniformer}} & S100-PM & 39.7 & \textbf{42.0} \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                       & 3Massiv & 42.8 & \textbf{43.6} \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                       & \abbrdataset & 50.2 & \textbf{50.4} \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{MViTv2-S\cite{li2022mvitv2}} & S100-PM & 36.9 & \textbf{41.0} \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                          & 3Massiv & 50.4 & \textbf{52.1} \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
                       % & \abbrdataset & 80.70 & 80.68 \\
                       & \abbrdataset & 61.7 & \textbf{62.0} \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline



\end{tabular}

==> tables/shape_crop_X3D.tex <==

\setlength{\tabcolsep}{2.0mm}
\begin{tabular}
{c | c | c c c}
\toprule
% Data & Model & 224$\times$224 & 256$\times$192 & 288$\times$192\\
% \arrayrulecolor{white}\cline{3-5}
% \arrayrulecolor{black}\cline{3-5}
% \arrayrulecolor{black}\cline{3-5}
% \arrayrulecolor{white}\cline{3-5}
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% \multirow{2}{*}{S100-PM} & Uniformer-S & 42.18 & 43.30 & 45.55 \\
% \arrayrulecolor{white}\cline{2-5}
% \arrayrulecolor{white}\cline{2-5}
% \arrayrulecolor{black}\cline{2-5}
% \arrayrulecolor{white}\cline{2-5}
% \arrayrulecolor{white}\cline{2-5}
%                        & MViTv2-S & 41.04 & 40.03 & 45.49 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% \multirow{2}{*}{3Massiv} & Uniformer-S & 44.75 & 45.24 & 46.87 \\
% \arrayrulecolor{white}\cline{2-5}
% \arrayrulecolor{white}\cline{2-5}
% \arrayrulecolor{black}\cline{2-5}
% \arrayrulecolor{white}\cline{2-5}
% \arrayrulecolor{white}\cline{2-5}
%                           & MViTv2-S & 52.08 & 52.30 & 53.78 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline

Model & Data & 256$\times$256 & 256$\times$192 & 288$\times$192\\
\arrayrulecolor{white}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{black}\cline{3-5}
\arrayrulecolor{white}\cline{3-5}
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
\multirow{2}{*}{X3D-M} & S100-PM & 53.09 & 51.95 & 52.38 \\
\arrayrulecolor{white}\cline{2-5}
\arrayrulecolor{white}\cline{2-5}
\arrayrulecolor{black}\cline{2-5}
\arrayrulecolor{white}\cline{2-5}
\arrayrulecolor{white}\cline{2-5}
                       & 3Massiv & 53.06 & 52.32 & 51.93 \\
\arrayrulecolor{white}\cline{2-5}
\arrayrulecolor{white}\cline{2-5}
\arrayrulecolor{black}\cline{2-5}
\arrayrulecolor{white}\cline{2-5}
\arrayrulecolor{white}\cline{2-5}
                       & \textcolor{red}{Ours} & 80.19 & 81.21 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline



\end{tabular}

==> tables/shape_crop_costs.tex <==

\setlength{\tabcolsep}{2.0mm}
\begin{tabular}
{c | c | c c c}
\toprule
% Data & Model & 224$\times$224 & 256$\times$192 & 288$\times$192\\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% \multirow{2}{*}{S100-PM} & Uniformer-S & 42.18 & 43.30 & 45.55 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
%                        & MViTv2-S & 41.04 & 40.03 & 45.49 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline
% \multirow{2}{*}{3Massiv} & Uniformer-S & 44.75 & 45.24 & 46.87 \\
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{black}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
% \arrayrulecolor{white}\cline{2-4}
%                           & MViTv2-S & 52.08 & 52.30 & 53.78 \\
% \arrayrulecolor{white}\hline
% \arrayrulecolor{black}\hline
% \arrayrulecolor{white}\hline

Model & 224$\times$224 & 256$\times$192 & 288$\times$192\\
% \multirow{2}{*}{Model} & \multirow{2}{*}{Data} & 224$\times$224 & 256$\times$192 &  288$\times$192 \\
  % &  & xxG & xxG & xxG \\
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{black}\cline{2-4}
\arrayrulecolor{white}\cline{2-4}
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
X3D-M & 51.97 & 51.60 & 50.75 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
Uniformer-S & 41.98 & 43.30 & 45.41 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline
MViTv2-S & 41.04 & 40.03 & 45.53 \\
\arrayrulecolor{white}\hline
\arrayrulecolor{black}\hline
\arrayrulecolor{white}\hline



\end{tabular}
